A registration method for reduced basis problems using linear optimal transport

We present a registration method for model reduction of parametric partial differential equations with dominating advection effects and moving features. Registration refers to the use of a parameter-dependent mapping to make the set of solutions to these equations more amicable for approximation using classical reduced basis methods. The proposed approach utilizes concepts from optimal transport theory, as we utilize Monge embeddings to construct these mappings in a purely data-driven way. The method relies on one interpretable hyper-parameter. We discuss how our approach relates to existing works that combine model order reduction and optimal transport theory. Numerical results are provided to demonstrate the effect of the registration. This includes a model problem where the solution is itself a probability density and one where it is not.

==> chapters/MoreNumericalExamples.tex <==
\section{Further results from the numerical experiments}\label{sec:more_numerical_examples}

In this section, we provide some more details and plots about the second numerical example considered in \cref{sec:numerical_examples}.

\subsection{Transport mappings}

Figure \ref{fig:xis_2} shows the first three transport modes and Figure \ref{fig:ws_2} depicts the corresponding weight functions $(t,\theta) \mapsto w_{1,2,3}(t,\theta)$. 
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.3\textwidth]{figs/ex2/xi1}
	\includegraphics[width=0.3\textwidth]{figs/ex2/xi2}
	\includegraphics[width=0.3\textwidth]{figs/ex2/xi3}
	\caption{First three transport modes with an added constant such that $\xi^c_{1,\dots,3}(0,0) = 0$.}
	\label{fig:xis_2}
\end{figure}
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.3\textwidth]{figs/ex2/w1}
	\includegraphics[width=0.3\textwidth]{figs/ex2/w2}
	\includegraphics[width=0.3\textwidth]{figs/ex2/w3}
	\caption{The Gaussian process approximation of the functions $w_{1,\dots,3}(t,\theta)$.}
	\label{fig:ws_2}
\end{figure}

\subsection{Approxmiation of the solution}

We repeat the procedure from \cref{sec:nonlinear_advection} for $\epsilon(\mathcal{E}) = 10^{-3}$ for the proposed method and compare it to the POD method without registration using $\epsilon(\mathcal{E}) = 10^{-6}$.  We can observe in \cref{fig:errs_ex2_2} that the $L^2$ error in the reduced method increases substantially (by a factor of $\approx 3$) in the first time-step. We believe that it is a result of the approximation of $\{ \partial_t w_j \}_{1 \leq j \leq m}$ through second-order centred finite differences, which becomes relevant once the resolution through the reduced basis is sufficient. We observed this behaviour in other (linear) time-dependent tests as well. In these cases, the error was an offset of the solution, i.e. $u_{\mathrm{rb}}(x) \approx u(x + \delta)$, where $| \delta |$ decreased with the time-step size.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.33\textwidth]{figs/ex2/L2err_nm=40_4_3}
	\includegraphics[width=0.33\textwidth]{figs/ex2/H1err_nm=40_4_3}
	\caption{Relative $L^2$- and $H^1$-errors for the non-linear advection-diffusion equation as a function of time. Plotted is the average error across all ten values of $\theta$. The shaded area is bounded above and below by the maximum and minimum error. Shown: $u_{\mathrm{trb}}$ with $\epsilon(\mathcal E) = 10^{-3}, n = 4, m=3$ and $u_{\mathrm{rb}}$ with $\epsilon(\mathcal E) = 10^{-6}, n = 40, m=0$.}
	\label{fig:errs_ex2_2}
\end{figure}
%\begin{table}[h!]
%	\centering
%	\begin{adjustbox}{width=1\textwidth}
	%		\begin{tabular}{ccc | ccc | ccc}
		%			$\epsilon(\mathcal{E})$ & $n$ & $m$ & \multicolumn{3}{c | }{relative $L^2$ error of $u(t=1.0,\theta)$ }  & \multicolumn{3}{c}{relative $H^1$ error of $u(t=1.0,\theta)$ } \\ \hline
		%			& & & avg & sd & max & avg & sd & max \\
		%			$10^{-4}$ & 26 & 0 & $5.30 \times 10^{-1}$ & $2.96 \times 10^{-1}$ & $8.48 \times 10^{-1}$ & $8.76 \times 10^{-1}$ & $4.77 \times 10^{-1}$ & $1.38 \times 10^{0}$ \\
		%			$10^{-6}$ & 40 & 0 & $5.28 \times 10^{-1}$ & $2.95 \times 10^{-2}$ & $8.45 \times 10^{-1}$ & $8.74 \times 10^{-1}$ & $4.82 \times 10^{-1}$ & $1.38 \times 10^{0}$ \\ \hline
		%			%				
		%			$10^{-2}$ & 3 & 2 & $1.19 \times 10^{-1}$ & $2.76 \times 10^{-2}$ & $1.53 \times 10^{-1}$ & $2.81 \times 10^{-1}$ & $4.10 \times 10^{-2}$ & $3.28 \times 10^{-1}$ \\
		%			$10^{-3}$ & 4 & 3 & $6.27 \times 10^{-2}$ & $2.52 \times 10^{-2}$ & $1.20 \times 10^{-1}$ & $1.72 \times 10^{-1}$ & $5.34 \times 10^{-2}$ & $2.95 \times 10^{-1}$ \\
		%			%
		%		\end{tabular}
	%	\end{adjustbox}
%	\caption{}
%	\label{}
%\end{table}


==> chapters/MoreOtherWorks.tex <==
\section{Further comparisons to other works}\label{sec:more_other_works}

This section recalls some more works on model order reduction and data compression based on OT techniques and discusses how they relate to our approach.

\subsection{Greedy barycenter approximation}

In \cite{ehrlacher_nonlinear_2020,battisti_waserstein_2022}, the authors apply barycentric approximations to one-dimensional PPDE problems. Using snapshots from a training set $\{ \rho(\mu_i) \}_{i=1}^{n_s}$, a collection of atoms is selected greedily. For every element of the training set, the best approximation using optimal barycentric coordinates given the present set of atoms is calculated. Then, the element of the training set with the largest approximation error is added as an additional atom until a set tolerance is reached. Assuming $n$ snapshots $\{ \rho(\mu_{i^1}), \dots, \rho(\mu_{i^n}) \}$ have been selected, one lets
\begin{equation}
	i^{n+1} = \argmax_{1 \leq i \leq n_s} \min_{\substack{\omega_1, \dots, \omega_n \geq 0 \\ \sum_{j=1}^n \omega_j = 1}} \mathrm{Loss} \left ( \rho(\mu_i), \mathrm{OTBar}(\omega_1, \dots, \omega_n; \rho(\mu_{i^1}), \dots, \rho(\mu_{i^n})) \right )
\end{equation}
and $\rho(\mu_{i^{n+1}})$ is added to the set of atoms. Once all atoms are determined, a mapping $\mu \mapsto \omega_1(\mu), \dots, \omega_n(\mu)$ is constructed by interpolation on the training set. The online phase now consists of evaluating this interpolating function and computing the corresponding barycentric approximation.

Since the examples in \cite{ehrlacher_nonlinear_2020,battisti_waserstein_2022} take place in one dimension, the calculations are greatly simplified. In fact, in one spatial dimension, there is a closed formula available for the transport from $\rho$ to $\sigma$, given by their cumulative distribution functions (cdf):
\begin{equation}
	T_{\rho \rightarrow \sigma} = \mathrm{cdf}(\sigma)^{[-1]} \circ \mathrm{cdf}(\rho).
\end{equation}
The superscript $^{[-1]}$ denotes the pseudo-inverse as defined in Chapter 2 of \cite{santambrogio_optimal_2015}. Note that for the case $\Omega = [0,1]$ and $\bar \rho = \mathbbm{1}_{[0,1]}$, the inverse cdf operation coincides with the Monge embedding: $T_{\bar \rho \rightarrow \sigma} = \mathrm{cdf}(\sigma)^{[-1]}$. Furthermore, the LOT barycenter in this case coincides with the OT barycenter:
\begin{equation}
	\mathrm{cdf} \circ \mathrm{OTBar}(\omega_1, \dots, \omega_n; \rho_1, \dots, \rho_n) = \left ( \sum_{i=1}^n \omega_i \mathrm{cdf}(\rho_i)^{[-1]} \right )^{[-1]}.
	%&= \mathrm{cdf} \circ \mathrm{LOTBar}^{\bar \rho = \mathbbm{1}_{[0,1]}}(\omega_1, \dots, \omega_n; \rho_1, \dots, \rho_n) \nonumber \\
\end{equation}

In \cite{ehrlacher_nonlinear_2020}, the authors also propose the method of \emph{tangent principal component analysis} (tPCA) on the set of $\{ \mathrm{cdf}(\rho(\mu_i))^{[-1]} \}_{i=1}^{n_s}$. This approach, which proved numerically unstable, is a special case of performing a POD on the Monge embeddings. The difference in our approach consists in the extension to arbitrary spatial dimensions, the use of a non-uniform reference density, and the introduction of entropic relaxation in order to increase the regularity of the transport maps.

\subsection{Sparse optimal transport barycenters}

In the recent work \cite{do_approximation_2023}, the method of barycenter encoding is extended by enforcing sparsity on the weight vectors. This is beneficial to memory footprint and run-time cost on the one hand, and mitigates issues of possible redundancy in the set of atoms on the other hand. In order to tackle problems in dimension $d > 1$, the barycenters are computed using entropic regularization. The online phase is again interpolating in nature, with novel methods provided to evaluate the mapping $\mu \mapsto \omega_1(\mu), \dots, \omega_n(\mu)$ based on local Euclidean embeddings. Importantly, the set of atoms selected in the online phase is now adaptive: given $\mu$, the atoms $\{ \rho(\mu_{i^1}), \dots, \rho(\mu_{i^n}) \} \subset \{ \rho(\mu_{i}), \dots, \rho(\mu_{n_s}) \}$ used to approximate $\rho(\mu)$ are chosen adaptively. In contrast, the greedy method from \cite{battisti_waserstein_2022,ehrlacher_nonlinear_2020} used the same $n$ atoms to approximate all $\rho(\mu)$. The adaptive method turns out to be not only cheaper to train than the greedy algorithm from by a factor of more than $10^{5}$, but also leads to more accurate reconstructions in numerical experiments.

In \cite{mueller_geometric_2022}, extending \cite{schmitz_wasserstein_2018}, the authors promote sparsity and uniqueness in the encoding by adding an additional term to the objective \eqref{eq:schmitz_barycenter_coordinates}, weighted by a balance parameter $\delta > 0$:
\begin{equation}
	\min_{\substack{\omega_j(\rho_i) \geq 0 \; \forall i,j \\ \sum_{i=j}^n \omega_j(\rho_i) = 1 \; \forall i \\ \sigma_1, \dots, \sigma_n \in \cP(\Omega)}} \sum_{i=1}^{n_s} \left ( \mathrm{Loss} \left ( \rho_i,  \mathrm{OTBar}( \{ \omega_j(\rho_i) \}_{j=1}^n; \{ \sigma_j \}_{j=1}^n ) \right ) \\ + \delta  \sum_{j=1}^n \omega_j(\rho_i) \OT(\rho_i, \sigma_j)^2 \right ).
\end{equation}
The problem as $\delta \rightarrow \infty$ is solved by binary assignment, where each weight vector $\{ \omega_j(\rho_i) \}_{j=1}^n$ has only one non-zero entry $\omega_{j*(\rho_i)} = 1 \;  \forall i$, corresponding to the nearest neighbour $\sigma_{j*}$ of $\rho_i$. \\

\subsection{Advection modes}\label{sec:advection_modes}

The registration method presented in \cite{iollo_advection_2014} uses OT techniques to build the mapping $\Phi_{\mu}$. Compared to the present work, there are three main differences: Firstly, the mapping of the snapshots is done in the sense of push-forward measures, that is
\begin{equation}
	\rho(\mu) \approx \left ( \bar \rho \circ \Phi_\mu + r(\mu) \circ \Phi_\mu  \right ) \det D\Phi_\mu 
\end{equation}
where $r(\mu)$ is a residual defined in the reference configuration. Note the presence of the Jacobian determinant of the mapping when compared to our formulation for $u_{\mathrm{trb}}$ in \eqref{eq:OTRB_approx}. As in the present work and as in \cite{taddei_registration_2020,taddei_space-time_2021} the residual is approximated by linear combinations of POD modes. The mapping is approximated as a linear combination of \emph{advection modes}, which are obtained using the distance matrix $\mathbb{D} := \{ \OT(\rho(\mu_i),\rho(\mu_j)) \}_{1 \leq i,j \leq n_s}$. In the case of an Euclidean distance, i.e. if one were to replace $\OT$ by $\Vert \cdot \Vert_2^2$, one could reconstruct the positions of $\rho(\mu_1),\dots, \rho(\mu_{n_s}) \in \bR^N$ up to rotations and translations of the entire set solely from the relative distance information contained in $\mathbb{D}$ by performing a singular value decomposition of the matrix $\mathbb{B} := - \tfrac{1}{2} \mathbb{J} \mathbb{D} \mathbb{J}$. Here, $\mathbb J = \mathrm{Id} - \tfrac{1}{n_s} \mathtt{1}\mathtt{1}^T$ and $\mathtt{1}$ denotes a vector of ones. Furthermore, retaining only the $m$ largest singular values, one can obtain the best approximate positions in an $m$-dimensional space. A comprehensive review of Euclidean distance matrix methods is given in \cite{dokmanic_euclidean_2015}.

For the OT distance, however, $\mathbb{B}$ is not positive semi-definite \cite{peyre_computational_2019}. By omitting the negative singular values, the authors obtain approximations of the positions of $\rho(\mu_1),\dots, \rho(\mu_{n_s}$ in a low-dimensional space. By inspection, they find parametrizations of $\mu \mapsto \Phi_\mu$. For example, if the reconstructed positions lie on a line, then the dominant advection mode is the transport map connecting the solution at its beginning to the one at the end.

The definition $u_{\mathrm{trb}}(\mu) = \sum_{i=1}^{n_m} \tilde u(\mu)_i \, \phi_i \circ \Phi_\mu$ used in our work corresponds to the push-forward of a function using $\Phi_\mu^{-1}$. The same operation is used to obtain the reference reduced basis. Especially in the case where $u$ itself is used to construct the transport mappings, one could also use the push-forward as applied on a density. In a sense, this is a natural choice, since the transport mappings are constructed to fulfil the push-forward relation for a density. Up to numerical inaccuracies, it holds on the training set that
\begin{equation}\label{eq:push_forward_mapping}
	\bar \rho = \rho(\mu_i) \circ \left ( \mathrm{id} - \nabla \psi^c(\mu_i) \right ) \det \left ( \mathrm{Id} - D^2 \psi^c(\mu_i) \right ) \quad \forall i = 1,\dots,n_s,
\end{equation}
and therefore the only reference reduced basis function is expected to be $\bar \rho / \Vert \bar \rho \Vert_{L^2}$.

We chose to not follow this approach for three reasons: First, relation \eqref{eq:push_forward_mapping} only holds if the transport mappings are constructed directly from $u$ itself and not another derived quantity. Second, mappings of the form $\phi \, \circ \, \Phi_\mu$ are used in standard finite element codes to go from a reference domain to the physical domain. These routines can then be utilized in the implementation. Third, substituting the push-forward relation for a density into a PDE residual requires evaluating derivatives of $\det \left ( \mathrm{Id} - D^2 \psi^c(\mu_i) \right )$, which requires even more regularity of $\psi^c$, and higher order basis functions in the discretization. \\






